GSNeRF: Generalizable Semantic Neural Radiance Fields with Enhanced 3D Scene Understanding

Utilizing multi-view inputs to synthesize novel-view images, Neural Radiance Fields (NeRF) have emerged as a popular research topic in 3D vision. In this work, we introduce a Generalizable Semantic Neural Radiance Field (GSNeRF), which uniquely takes image semantics into the synthesis process so that both novel view images and the associated semantic maps can be produced for unseen scenes. Our GSNeRF is composed of two stages: Semantic Geo-Reasoning and Depth-Guided Visual rendering. The former is able to observe multi-view image inputs to extract semantic and geometry features from a scene. Guided by the resulting image geometry information, the latter performs both image and semantic rendering with improved performances. Our experiments not only confirm that GSNeRF performs favorably against prior works on both novel-view image and semantic segmentation synthesis but the effectiveness of our sampling strategy for visual rendering is further verified.

==> Figure/compare_geonerf.tex <==
\begin{figure}[t]
% \Huge
\resizebox{\linewidth}{!}{%

\begin{tabular}{ccc}
 
 {\fontsize{30}{36}\selectfont GT} &
 {\fontsize{30}{36}\selectfont GeoNeRF + semhead} & 
 {\fontsize{30}{36}\selectfont GSNeRF (Ours)}\\
 
\includegraphics[]{Figure/qualitative/45/45_image_GT.jpg} &
\includegraphics[]{Figure/qualitative/GeoNeRF_45/00124954_2447_image_pred.jpg} &
\includegraphics[]{Figure/qualitative/45/45_image_pred.jpg} \\


\includegraphics[]{Figure/qualitative/45/45_semantic_GT.jpg}  & 
\includegraphics[]{Figure/qualitative/GeoNeRF_45/00124954_2447_semantic_pred.jpg} &
\includegraphics[]{Figure/qualitative/45/45_semantic_pred.jpg} \\

 
\end{tabular}}


% \vspace{-3mm}
\caption{\textbf{Qualitative comparisons with GeoNeRF with semhead on ScanNet.} \frank{We compare the visual quality of the rendered novel view image and its semantic segmentation map with semantic-extend-version GeoNeRF~\cite{johari2022geonerf}.}
% \textcolor{brown}{should we add PSNR/mIOU numbers on the pictures or in caption?}
}
\label{fig:geonerf_compare}
\vspace{-0mm}
\end{figure}


==> Table/different.tex <==
% \renewcommand{\arraystretch}{1.3}% Wider
\begin{table}[t]
\centering
\resizebox{0.65\linewidth}{!}{%
\begin{tabular}{ccccc}
\hline
K & mIoU & acc. & class acc. & PSNR \\ \hline
4 & 48.70 & 72.71 & 57.97 & 31.02 \\
6 & 51.61 & 73.92 & 59.45 & 30.96 \\
8 & \textbf{58.30} & \textbf{79.79} & \textbf{65.93} & \textbf{31.33} \\ \hline
\end{tabular}}
\caption{\textbf{Comparisons of different source view numbers on ScanNet. } Note that $K$ indicates the number of source views used for training and testing.}
\label{different}
% \vspace{-2mm}
\end{table}

==> Table/finetune_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand{\arraystretch}{1.3}% Wider
\begin{table}[t]
\resizebox{1\linewidth}{!}{%
\begin{tabular}{l|cl|ccc}
\multirow{2}{*}{Finetuned Method} & \multicolumn{2}{c|}{GT Depth} & \multicolumn{3}{c}{ScanNet} \\ \cline{2-6} 
 & \multicolumn{2}{c|}{Train / Test} & mIoU & acc. / class acc. & PSNR \\ \hline
S-Ray & \multicolumn{2}{c|}{\cmark / \cmark} & 92.4 & 98.2 / 93.8 & 27.67 \\
Ours & \multicolumn{2}{c|}{\cmark / \,\,\,\,\,\,} & \textbf{93.9} & \textbf{99.1} / \textbf{98.4} & \textbf{31.70} \\ \hline
S-Ray & \multicolumn{2}{c|}{/\,\,} & 91.6 & 97.3 / 92.2 & 27.31 \\
Ours & \multicolumn{2}{c|}{/\,\,} & \textbf{93.2} & \textbf{98.2} / \textbf{96.8} & \textbf{30.89}

\end{tabular}}
\caption{\textbf{Results of finetuning on unseen scenes in ScanNet. } Note that methods in the first two rows take GT depth during training, while S-Ray additionally requires such inputs during testing. The methods in the last two rows do not have access to GT depth during training/testing.}
\label{finetune_table}
% \vspace{-2mm}
\end{table}
